An Approach to Causal Inference over Stochastic Networks

Claiming causal inferences in network settings necessitates careful consideration of the often complex dependency between outcomes for actors. Of particular importance are treatment spillover or outcome interference effects. We consider causal inference when the actors are connected via an underlying network structure. Our key contribution is a model for causality when the underlying network is unobserved and the actor covariates evolve stochastically over time. We develop a joint model for the relational and covariate generating process that avoids restrictive separability assumptions and deterministic network assumptions that do not hold in the majority of social network settings of interest. Our framework utilizes the highly general class of Exponential-family Random Network models (ERNM) of which Markov Random Fields (MRF) and Exponential-family Random Graph models (ERGM) are special cases. We present potential outcome based inference within a Bayesian framework, and propose a simple modification to the exchange algorithm to allow for sampling from ERNM posteriors. We present results of a simulation study demonstrating the validity of the approach. Finally, we demonstrate the value of the framework in a case-study of smoking over time in the context of adolescent friendship networks.

==> prelim.tex <==
\title{An Approach to Causal Inference over Stochastic Networks}

% List abbreviations here, if any. Please note that it is preferred that abbreviations be defined at the first instance they appear in the text, rather than creating an abbreviations list.
%\abbrevs{DAG, Directed Acyclic Graph; ERGM, Exponential-Family Random Graph Models; ERNM, Exponential-family Random Network Models; MRF, Markov Random Field; MCMC, Markov Chain Monte Carlo}

% Include full author names and degrees, when required by the journal.
% Use the \authfn to add symbols for additional footnotes and present addresses, if any. Usually start with 1 for notes about author contributions; then continuing with 2 etc if any author has a different present address.
\author[Duncan A. Clark]{Duncan A. Clark}
% \address{Duncan A. Clark, Department Of Statistics, University of California, Los Angeles, California, 90095}
\address{University of California - Los Angeles, Los Angeles, USA}
\email{duncanclark@ucla.edu}

\author[Mark S. Handcock]{Mark S. Handcock}
\address{University of California - Los Angeles, Los Angeles, USA}

% \presentadd[\authfn{2}]{Department, Institution, City, State or Province, Postal Code, Country}

%\fundinginfo{This article is based upon work supported by the National Science Foundation(NSF, MMS-0851555, SES-1357619, IIS-1546259) and National Institute of Child Health and Human Development (NICHD, R21HD063000, R21HD075714 and R24-HD041022). The content is solely the responsibility of the authors and do not necessarily represent the official views of the National Institutes of Health or the National Science Foundation.}

% Include the name of the author that should appear in the running header
% \runningauthor{Author One et al.}
